Opportunistic Device-to-Device Communication in Cellular networks: From Theory to Practice

This dissertation studies different aspects of D2D communications and its impact on the key performance indicators of the network. We design an architecture for the collaboration of cellular users by means of timely exploited D2D opportunities. We begin by presenting the analytical study on opportunistic outband D2D communications. The study reveals the great potential of opportunistic outband D2D communications for enhancing energy efficiency, fairness, and capacity of cellular networks when groups of D2D users can be form and managed in the cellular network. Then we introduce a protocol that is compatible with the latest release of IEEE and 3GPP standards and allows for implementation of our proposal in a today's cellular network. To validate our analytical findings, we use our experimental Software Defined Radio (SDR)-based testbed to further study our proposal in a real world scenario. The experimental results confirm the outstanding potential of opportunistic outband D2D communications. Finally, we investigate the performance merits and disadvantages of different D2D modes. Our investigation reveals, despite the common belief, that all D2D modes are complementary and their merits are scenario based.

==> 00-headers/acks_copy.tex <==
\chapter*{Acknowledgements}
\addcontentsline{toc}{chapter}{Acknowledgements}


First and foremost I want to thank my advisor Vincenzo Mancuso. It has been an honor to be his first Ph.D. student.  I appreciate all his contributions, the late nights that he spent reviewing my papers, funding to make my Ph.D. experience productive and stimulating, and insightful discussions about my research.
I also have to thank the members of my PhD committee, Professors XXX, XXXX, and XXXX for their helpful career advice and suggestions in general.

My special thanks goes to my other Ph.D. fellows, Ignacio De Castro Arribas, Thomas Nitsche and Qing Wang with whom I had long meeting in our favorite meeting room (a.k.a, kitchen). I am grateful to Christian Vitale and Vincenzo Sciancalepore for their collaborations. 

I will forever be thankful to my life partner, Allyson Sim, whose support and enthusiasm was vital to my progress within past 6 years. I hope I can return her support and kindness for years to come. 

Finally, but by no means least, thanks go to mum, dad and my sister for almost unbelievable support. They are the most important people in my world and I dedicate this thesis to them.
